FEDEX: An Explainability Framework for Data Exploration Steps

When exploring a new dataset, Data Scientists often apply analysis queries, look for insights in the resulting dataframe, and repeat to apply further queries. We propose in this paper a novel solution that assists data scientists in this laborious process. In a nutshell, our solution pinpoints the most interesting (sets of) rows in each obtained dataframe. Uniquely, our definition of interest is based on the contribution of each row to the interestingness of different columns of the entire dataframe, which, in turn, is defined using standard measures such as diversity and exceptionality. Intuitively, interesting rows are ones that explain why (some column of) the analysis query result is interesting as a whole. Rows are correlated in their contribution and so the interesting score for a set of rows may not be directly computed based on that of individual rows. We address the resulting computational challenge by restricting attention to semantically-related sets, based on multiple notions of semantic relatedness; these sets serve as more informative explanations. Our experimental study across multiple real-world datasets shows the usefulness of our system in various scenarios.

==> characterization.tex <==
\section{Interestingness Measures}
\subsection{Exceptionality Measure}
Exceptionality measure favors operations whose result views (\(V_{k+1}\)) deviates significantly from the previous view \(V_k\). we define the probability distribution \(P^k_A\) of view \(V_k\) and attribute \(A\) to be the relative frequency of it's values(i.e for every \(v \in V_k[A], p(v)\) is the probability to choose v uniformly). The definition of Exceptionality Measure of two views \(V_{k}, V_{k+1}\) and of specific attribute \(A\) is:
\begin{center}
\(Exceptionality(V_{k},V_{k+1}, A) = KL(P^k_A, P^{k+1}_A)\)    
\end{center}
Where \(KL\) is Kullback-Leibler divergence.
\subsection{Diversity Measure}
Diversity measure favors operations that their source and result view have notable differences in their values. The definition of Diversity Measure of two views \(V_{k}, V_{k+1}\) for specific attribute A is:
\begin{center}
\(Diversity(V_{k},V_{k+1}, A) = \frac{Var(P^{k+1}_A)}{Var(P^k_A)}\)
\end{center}
\subsection{Conciseness Measure}
Conciseness measure is defined differently for group by operations and other operations. In the case the view is grouped, the measure takes into account the number of groups, the number of attributes that are currently grouped by, the number of the underlying tuples, denoted \(g,a\), and \(r\) (respectively):
\begin{center}
\(Conciseness(V_{k}, A) = \frac{h(g\cdot a)}{h(r)}\)
\end{center}
where \(h(\cdot)\) is a normalized sigmoid function with a predefined width and center. In case \(V_{k}\) is not grouped, the measure is:
\begin{center}
\(Conciseness(V_{k}, V_{k+1}, A)  = h(\frac{r_k}{r_{k+1}})\)
\end{center}
where \(r_k, r_{k+1}\) are the number of tuples in \(V_{k}, V_{k+1}\) (respectively).
\subsection{Verbosity Measure}
Unlike all the measures we introduced, this measure can be applied only to Join operation (with two source views) and relevant only to the join attribute(the attribute the join operation calculated by). Verbosity measure is high when the source views are "highly joinable". The measure is taken from JOSIE paper\cite{JOSIE}, and is very intuitive:
\begin{center}
\(Verbosity(V_{1}, V_{2}, A)  = \frac{|V_{1}^{A} \cup V_{2}^A|}{|V_{1}^{A}|}\)
\end{center}
where \(V_{i}^{A}\) is the set of values of attribute \(A\) in view \(V_{i}\), and \(|\cdot |\) is the size of the set. 
\section{Non-Relative Measures}
Not all interestingness measures are calculated relatively, For instance, some times an operation creates a "new" attribute, which cannot be compared to a corresponding attribute at the previous view. Some measures (like Verbosity Measure) simply cannot be calculated relatively (no previous reference view exists).
\subsection{Diversity Measure for Group By Operations (Special Case)}
For Group by operations, we cannot examine a relative interestingness of the aggregated attributes, because they changes dramatically and will be very different from the previous view's attribute values. So we have to omit it:
\begin{center}
\(Diversity(V_{k+1}, A) = Var(P^{k+1}_A)\)
\end{center}
Because of this little change, we consider it as an entirely different measure, because we cannot compare between two different formulas, with different distribution of values, as they were one. (We compare measure values when we calculate the view measure on section 4, by choosing the attribute that maximizes the attribute measure)
\section{Interestingness Measure for Views}
\subsection{Single Source View}
Given an attribute measure \(M(V_1, V_2, A)\) we define view measure \(M(V_1,V_2)\) as the maximal attribute measure:
\begin{center}
\(M_{view}(V_{k},V_{k+1}) = \max_{A \in Attr}(M(V_{k},V_{k+1}, A))\)
\end{center}
notice that both Diversity measure and Exceptionality measure match this measure pattern. for Group by operation the \(Attr\) group contains only the aggregated attributes.
\subsection{Multiple Source Views}
The above views measure cannot apply to all operations - for instance for the Join operation - because we have more than one source view. specifically for join, there are two types of attributes - 1. mutual attributes- the attributes the join operation is calculated by, which must be at both source tables, and 2. unique attributes- the other attributes, which must not be at both source tables, or must be renamed. for simplicity we assume that all those attributes have different names (we can always rename the attributes in a separate operation). In order to generalize the Measure calculation for Join operations and another operations with more than one source views, we introduce a better version of the previous view measure -
 
\begin{center}
\(M_{view}(\{V\}_{i=1}^k, V') := \max_{A \in V'}(\min_{\{V_i | A \in V_i\}}(M(V^i, V',A))\)
\end{center}

where  \(V_1, V_2, \cdots,V_k\) are the source views and \(V'\) is the result view.
notice that for unique attributes, the change in the formula above changes nothing in the result. But for mutual attributes, the result is the minimum view measure from all source views. In this way we check the interestingness between source and result view, and not source and source views (the result view may be dependent heavily on one source view only, for instance Join operation of two tables T1,T2 by some index attribute A - which is our "mutual attribute" - where \(T1.A\subset T2.A\). It easy to notice that in this case the result view is dependent entirely on \(T1.A\)) 
\subsection{Grouping of Columns with high correlation}
Sometimes a dataset contains two or more columns which has a very high correlation, sometimes even by definition. For instance - salary and taxes paid or male, female, and unisex columns of some measure as age, height, etc. are highly correlated by definition. Such attributes gets often very high correlation score at measures such as Pearson/Kendall Tau correlation coefficient, or Spearman rank correlation coefficient. To summarize and improve efficiency, we add a group phase before calculating the interestingness measure and it's corresponding shapley values. In this phase we calculate which columns are highly correlated (for example by setting some correlation coefficient and a threshold), grouping them into groups of correlated columns, and then pick one of them to be the representative of the group, dropping all the rest. While we do not calculate interestingness measures and shapley values for those columns, we can add them to the explanation if their representative column is the chosen column for the interestingness NL explanation.
\subsection{Comparing Different Interestingness Measures}
Different Interestingness measures have different values distribution. comparing them as-is will give wrong results, and maybe even predictable result each time, if some measure output values are always higher than other measures. Hence we have to normalize the scores to distribute the same, and just then compare them to find the highest interestingness measure w.r.t the current view. For this issue we use work done by \cite{Interestingness}, which suggest such approach of normalizing such interestingness measures. 
\section{Relative Measures for Shapley Values}
Given a result view \(V'\), and an attribute \(A\) that maximized some view measure \(M\), The contribution of a set \(S \subseteq V'[attr]=S\cup S'\) is defined as:
\begin{center}
\(\phi(S):=M(V[A]\setminus S', V'[A]\setminus S', A)\)
\end{center}
This calculation holds for both Exceptionality measure and Diversity measure, and is expandable to more measure of the same structure.
\section{Interesting measure vs. explainable measure}
To explain why a view is interesting, we use interestingness measures, as shown above. Every measure comes with corresponding NL pattern, which can explain why some view is interesting, and should explain why this interestingness measure got high score. In this paper we suggested Shapley value to determine which records influenced the result the most, w.r.t some interestingness measure. While this should explain why the view is interesting, it will success to summarize the explanation only if some records highly influence the final interestingness score. If, for some reason, all of the records influence the interestingness score the same, showing some of them gives absolutely no insight or explanation why the score is high, or why the view is interesting. To summarize - we have two cases - 1. The view is interesting and some records summarize why the entire view is interesting, and 2. The view is interesting, but we cannot explain why it is interesting using only a small set of the view's records.

Hence we can suggest a new measure, this time this measure measures the interestingness measure - whether it is explainable or not. Given an array of shapley values of the result view's records, we compute the explainability of an interestingness measure as the variance of the shapley values-
\begin{center}
    \(Explainability(shap\_array) := Var(shap\_ array)\)
\end{center}
It is highly important to calculate the shapley values with the normalized interestingness function as the target function, otherwise the results will be biased to the score with the higher values.
Now, given an interestingness measure and it's explainability score, we define an elaborate score, to be the product of both measures. this way we pick high interestingness measure which is also explainable.

\subsection{Correlation Influence on explainability}

When performing an operation \(Op\) on some column \(A\), Interestingness measures tend to have high value for columns with high correlation with the column A. Lets assume some column \(B\) has very high correlation with column \(A\), It make sense that column \(B\) will have high interestingness score because measures like Exceptionality and Diversity will spot a high difference in the distribution of column \(B\) values, unlike other columns with very low correlation, which will appear to have changes that look random, and hence changes in their values distribution will be minor.
In such case, the Explainability score will be lower than usual, because most of the values in the result view will contribute equally to the interestingness score, because they mirror the changes in column \(A\) distribution on some other column \(B\). In practice, in our experiments we noticed that Explainability-Correlation tend to be inverse proportional to each other- high correlation means low explainability and vice versa.

\section{Example}
We used the dataset "summer-products-with-rating-and-performance\_2020-08.csv", which describes summer products selling in 2020. This dataset contains 42 columns, but our explanation focused only on small part of them: 
units\_sold - how many items of this product sold. rating - number between 1 and 5 describing the rating of the product(filled by buyers). rating\_count - number of buyers that rated the product. merchant\_rating - the rating of the merchant who sells this product. merchant\_rating\_count - number of buyers that rated the merchant.

We performed a filter operation and inspected it via the Exceptionality measure, in order to show the relation between the measure score, the Explainability, and the correlation. The operation is:
\(Filter("units\_sold", <=, 50) )\).
The column with the highest score was "rating\_count", with Exceptionality score of 0.81. Even that this is the most "interesting" thing about this view, the explanation is not enlightening: "current view shows high exceptionality, specifically, the major deviation occurs on the attribute "rating\_count" with relation to table "summer\_products". For instance- the probability of rating\_count values between 2.00 and 4.00 was 0.042 and changed to 0.277...". In first glance it's look like a big difference, but in second thought - if there are not much units sold, it is obvious that the rating count will be low too. But if we'll look at the correlation, we see that units\_sold and rating\_count have very high correlation - of 90\%!, and, as we will see, the shapley variation is lower then other columns - 0.0002. 

After this case, if we'll take a look at the second best- "merchant\_rating\_count", now with much lower Exceptionality score of 0.45. The explanation now is a little bit more enlightening - "... the probability of merchant\_rating\_count values below 56.05 was 0.046 and changed to 0.213, the probability of merchant\_rating\_count values between 56.05 and 181.36 was 0.046 and changed to 0.191 ..." - we can see that merchants with unpopular product are usually unpopular. In this case, the correlation is already much lower - 26\%, and the shapley values variation is much higher - 0.0011. 
The third most interesting column, after rating\_count and merchant\_rating\_count, is "rating". The explanation generated by our engine is: "... the probability of rating values above 4.90 was 0.046 and changed to 0.362 ...". We can conduct that unpopular products often have very high rating. The correlation now is very low - only 6\%, and the shapley variation is 0.0001, which is close to the first explanation. 
In conclusion, we can see that while "rating" column got the highest score, it is somehow the least interesting column out of those three columns. Hence we can improve our explanation selection by looking at the correlation and the Explainability of an explanation, and not only by the interestingness measure itself. 


==> introduction.tex <==
\section{Introduction}\label{sec:intro}
%\amit{ important: (1) stress who's the client - (2) break the solution to interestingnes and contribution}

% \amit{we are the first system the doesnt explain only a dataframe but regards the entier step. I.e., what subsets of the input dataframe, made impact on the output dataframe}
% \ag{To the best of our knowledge, this is the first approach that automatically generates explanations for output dataframes in the context of the of the exploratory step, i.e., the input dataframe and the operation itself.}


Exploratory Data Analysis (EDA) is an essential process performed by data scientists and analysts in order to up-close examine a new dataset, better understand its nature and characteristics, and extract preliminary insights from it. 
EDA is typically performed in \textit{scientific notebooks}~\cite{kery2018story} using a dataframe library~\cite{reback2020pandas} which allows users to interactively transform and analyze datasets via programmatic query operations (such as filter, aggregation, join, pivot, etc). 
In each exploratory step, the analyst runs a query over the previously obtained dataframe, examines the resulting dataframe to derive intermediate insights, and decides on the next exploratory step. 

%The notebook interface also allows users to document their exploration process and highlight their insights using data visualizations and accompanied text.

EDA is a challenging process, where arguably the most significant challenge lies in scanning the (possibly many) query results obtained in each step to identify interesting patterns and trends. These discoveries are crucial both for gathering insights and conceiving the next exploratory steps.  
To illustrate the difficulty faced by analysts in interpreting the results of exploratory steps, consider the following example EDA scenario. 


%\amit{why is this helpful? why is it challenging? - stress that it is important for gathering inermediate insights and also to decide which operations to employ next}
%In this research we focus on the latter challenge, which is particularly time-consuming, as analyzing such exploratory 
%by carefully examine thousands of tuples, perform subsequent transformations, and compose visualizations.  


%To assist users in analyzing and understanding their exploration steps,
%To this end, we suggest \sys{}, an interactive framework that automatically \textit{explains} exploratory steps and highlights their interesting elements using easy-to-read captioned visualizations. This allows users to quickly gain insights from each exploratory steps they perform.

%First, to illustrate the difficulties in understanding   \sys{}.

%\subsection{Example Exploration Process with explanations}




\begin{comment}
\begin{figure}[t]
\vspace{-3mm}
    \centering
    \includegraphics[scale = 0.28, trim = 0 0 0mm 0mm]{images/explainer.png}
    \caption{\sys\ Architecture}
    \label{fig:framework}
\end{figure}
\end{comment}

\begin{figure*}[t!]
\centering
%\begin{subfigure}[t]{0.45\textwidth}
\begin{subfigure}[t]{0.7\textwidth}
    \fbox{\includegraphics[width=0.98\linewidth]{{images/spotify_filter2.pdf}}}
        %\vspace{-6mm}
        \caption{Filter results}
        \label{fig:spotify_filter}
        %\vspace{-5mm}
\end{subfigure}
~~~
\begin{subfigure}[t]{0.25\textwidth}
    \fbox{\includegraphics[width=0.87\linewidth]{{images/spotify_groupby2.pdf}}}
        %\vspace{-1mm}
        \caption{Group-by results}
        \label{fig:spotify_groupby}
        %\vspace{-3mm}
    \end{subfigure}
%    \vspace{-3mm}
    \caption{\linespread{1}\selectfont{} \textbf{Result samples of filter and group-by operations over the Spotify ``Song Popularity Dataset''.} \normalfont{Figure~\ref{fig:spotify_filter} shows partial results of a filter operation that leaves in only songs with `popularity' scores above 65. Figure~\ref{fig:spotify_groupby} depicts partial results of a group-by operation, showing for each year -- since 1990 -- the mean `loudness' and `danceability' values.}}
    \label{fig:spotify}
\end{figure*}

\begin{figure*}[t]
\centering
\begin{subfigure}[b]{0.49\textwidth}
\fbox{\includegraphics[width=0.92\linewidth]{{images/explanation_filter.pdf}}}
\vspace{-2mm}
    \caption{Explanation for the filter step (Figure~\ref{fig:spotify_filter})}
    \label{fig:explained_filter}
    \end{subfigure}
    %\skip
    \hspace*{\fill}
\begin{subfigure}[b]{0.49\textwidth}
\vspace{-51mm}
    \fbox{\includegraphics[width=0.99\linewidth]{{images/explanation_groupby.pdf}}\vspace{8mm}}%, trim={0 6mm 0 0}
    \vspace{-2mm}
     \caption{Explanation for the group-by step (Figure~\ref{fig:spotify_groupby})}
     \label{fig:explained_groupby}
    \end{subfigure}
    \caption{  \textbf{Multi-modal explanations generated by \sys{}.} \normalfont{Figure~\ref{fig:explained_filter} explains the Spotify filter results, showing songs with popularity scores above 65. Our framework has identified that the highest contribution to the interestingness score is due to songs made in the 2010s --  they form 61\% of the popular songs, compared to only 3.5\% in the entire dataset, leading to the insight that \underline{\textit{new songs tend to be more popular than older songs}}}. Figure~\ref{fig:explained_groupby} explains the Spotify group-by results, showing mean `loudness' and `danceability' values for each year. Our explanation employs a many-to-one partition (see Section~\ref{sec:binning}), and points out that \underline{\textit{songs made in the 90's tend to be less loud than later songs}}.} 
    \label{fig:explained_new}
\end{figure*}








%which is to analyze the resulted view, at each step of the exploratory process, and \textit{draw insights and conclusions} from it. To that end, we suggest developing an explainability framework for EDA processes, that will inspect users' EDA operations and automatically highlight the key elements in the resulted views that made them interesting. The explanations will be provided in an intuitive, bimodal manner that combines a natural-language phrase and compatible visualizations, altogether geared to bring to the surface coherent insights. 
% \paragraph*{Example Exploration Process }
\begin{example}\label{ex:spotify-eda}
Data scientist Clarice works on a dataset of song information, published by Spotify~\cite{spotifydataset}.
%, with the goal of understanding \textit{what makes songs popular}.

The dataset (see samples in Figure~\ref{fig:spotify}) contains a \textit{popularity score} for each song, alongside 37 descriptive features  (e.g., artist name, year, decade) as well as audio-analysis features such as \textit{loudness}, \textit{valence}, \textit{danceability} and others. 

\revb{Clarice is first interested in the question ``what makes songs popular?''. She therefore composes a filter operation showing songs that have a \textit{high} popularity score ($>65$).} Applying this operation yields a dataframe with 7000 rows and 37 columns (See Figure~\ref{fig:spotify_filter} for a small sample). Clarice now needs to examine these results in order to understand what is interesting about them. One such notion of interestingness may be captured by the question ``In what way are these popular songs different than the rest of the songs in the dataset?" To answer this question, Clarice needs to sift through the rows, apply additional data transformations, and generate data visualizations.


\revb{Clarice then decides to focus her analysis only on recent songs (released after 1990) and investigate their characteristics. 
To do so, she first filters the original dataframe to output songs released after 1990,
then performs a group-by to view the mean \textit{loudness} and \textit{danceability} values for each year.} A sample of the result of this group-by step appears in Figure~\ref{fig:spotify_groupby}. This step results in a much smaller dataframe than before, 
including about 30 rows and 3 columns. However, interesting patterns and trends are still not clearly visible -- are there any particular years with more `quiet' songs than the other? is there a trend where newer songs are more `loud' and `danceable'? Answering these questions still requires a substantial effort.  
\end{example}
%See that even for this much smaller dataframe, containing about 30 rows and 3 columns, the patterns and trends are still not obvious, thus requires time and effort to identify them and gather insights.  \qed{} 

%Understanding what is interesting in the results of the second, auto-generated operation is especially difficult, as Clarice may not immediately understand the nature of the operation (i.e., why did the system suggest filtering by ``$year~>=~1990$'', or select these specific attributes for group-by).
   

%Had Clarice used an EDA recommender system at this point, she would have obtained a next-step recommendation such as Group-by over the \textit{year} attribute, that shows the mean values for the numerical attributes \textit{loundness} and \textit{\textit{danceability}} for songs created after 1990 (See Figure~\ref{fig:spotify_groupby} for a snapshot). 
%Also for the second operation, gathering concrete insights is not easy. Especially if Clarice does not understand the operation iteself (e.g. why did the system suggest filtering by ``$year~>=~1990$''?)

% \vspace{2mm}


In this paper, we present \sys{} (Ef{\bf f}ici{\bf e}nt {\bf D}ata Exploration {\bf Ex}planations), an EDA explanation framework that assists users in analyzing and understanding the results of their exploration steps. \sys{} explains exploratory steps using a twofold process: (1) as an analyst would do, \sys{} inspects the resulted dataframe, and discover interesting aspects of it. For example, does it show outliers? Or perhaps a highly diverse set of values in one of the columns?; (2) since naturally, not all underlying tuples equally contribute to the interesting pattern discovered, \sys{} detects which data subsets \textit{cause} the resulted dataframe to be interesting. Therefore, a good \textit{explanation} for an exploratory step is a set-of-rows from the dataframe which \textit{significantly contributes} to a \textit{highly interesting} aspect of the results dataframe.  
Importantly, \sys{} tailors the explanation to the {\em context} of the generated dataframe, i.e., the EDA operation or query and the source dataframe.
\sys{} then presents this set-of-rows in a hybrid format via the notebook interface as coherent, easy-to-read \textit{captioned visualizations}. This allows users to quickly understand and derive immediate insights from each exploratory step they make. 
% presents this set-of-rows in a hybrid format that includes both a visualization that emphasizes the interesting trend in the data, and as a textual explanation that accompanies the visualization and allows for a better and faster understanding of the explanation. 
% The best such explanations are returned to the user via the notebook interface as coherent, easy-to-read \textit{captioned visualizations}, which allow users to quickly understand and derive immediate insights from each exploratory steps they make.  
% Consider the following example, illustrating the explanations generated by \sys{}.
The following example illustrates the explanations generated by \sys{}.

\begin{example}[\sys\ Explanations]\label{ex:explanations}
Figure~\ref{fig:explained_new} shows the explanations produced by \sys{}, for the two exploratory steps on the Spotify dataset in Example \ref{ex:spotify-eda} (see Figure~\ref{fig:spotify}). 
For the filter step, which focuses only on songs with popularity score greater than 65, \sys{} detects that in the `decade' column there exists a high, interesting \textit{deviation} from the input dataframe (namely, the dataframe Clarice applied the filter on). It then detects that most of the deviation is due to \textit{songs from the \textit2010s}. Using a side-by-side bar plot, \sys{} highlights the difference in the number of songs from the 2010s decade before and after the filter, showing that \textit{newer songs from the last decade tend to be more popular than older songs}. 
As for the group-by step, showing the mean `loudness' and `danceability' values for each release year, \sys{} identifies an interesting pattern in the column `loudness', whose values greatly differ from one another. It then detects that the large diversity in values occurs mainly due to years in `1990s', highlighting that \textit{the songs released in the 1990s are significantly less loud than songs made in later years}. 
% \qed{} 
\end{example}


Previous work has proposed a multitude of approaches for assisting data exploration,
such as recommending next exploratory steps~\cite{Somech2018REACTKDD,seleznova2020guided},
query auto-completion~\cite{khoussainova2010snipsuggest,le2019explique}, visualization~\cite{VartakRMPP15,lee2021lux,wongsuphasawat2016voyager} and even insights~\cite{tang2017extracting,asudeh2020detecting} recommendations. While all of these works indeed reduce the manual effort of composing queries, and even point users to some arbitrary interesting aspects of the data, they are not geared towards analyzing and explaining the results of users' exploration steps. 
% Our approach complements these works by providing explanations for the operations themselves and focuses users attention on the interesting part of the view w.r.t. the operation that created it.
However, to the best of our knowledge, \sys\ is the first system to automatically generates explanations for output dataframes {\em in the context of the exploratory step.}


%As the notebook interface allows for automatically creating visualizations and textual documentation, 

% The best such explanations are returned to the user via the notebook interface as coherent, easy-to-read \textit{captioned visualizations}, which allow users to quickly understand and derive immediate insights from each exploratory steps they make.  


\begin{figure*}[t]
\vspace{-3mm}
    \centering
    \includegraphics[width=0.9\linewidth]{images/drarft_architecture.pdf}
    \caption{\sys\ architecture}
    \label{fig:framework}
\end{figure*}





%\sys{} detects interesting facets in the queries' results, then compose corresponding explanations by 
%identifying which subsets of the dataframes cause an interesting phenomenon in the results. The best such explanations are returned to the user as coherent, easy-to-read \textit{captioned visualizations}, which allow users to quickly understand and derive immediate insights from each exploratory steps they make.  






% \vspace{2mm}






%detect data subsets that \textit{cause} the resulted dataframe to be interesting (Surely, not all underlying tuples equally contribute to the interesting pattern).


%Last, after detecting why and what exactly is interesting in the results, \sys{} is required to formulate a \textit{coherent explanation} that illustrates the discovered phenomena as clearly as possible .  







%\amit{required is not suitable -- we need to (1) discover what is interseting and (2) explain why it is interesting.}
%\amit{stress that it is not enough, as we show in the experiments - to only detect what is interesting. The user needs focus}

%This example scenario also shed some light about the required  
%This example scenario not only illustrates the users' difficulty in analyzing and drawing insights from each exploratory step, but also implies the challenges in designing our framework. 
%Exactly as the analyst would do, \sys{} first needs to inspect the resulted dataframe, and 
%discover interesting aspects of it. For example, does it show outliers? Or perhaps a highly diverse set of values in one of the columns? The second challenge is to detect data subsets that \textit{cause} the resulted dataframe to be interesting (Surely, not all underlying tuples equally contribute to the interesting pattern). Last, after detecting why and what exactly is interesting in the results, \sys{} is required to formulate a \textit{coherent explanation} that illustrates the discovered phenomena as clearly as possible .  

%\amit{now refer to the numbers - 1 computating what is interesting, 2 explaining why is it interesting - by computing the contribution. Explanation is defined as the set of rows which contributs to the interestingnss. How contribution is defined? - using intervention.}
%\amit{here this is a good place to say that one colud compute the interstingness and focus the the user on the intersetrintgness aspect. Yet this is not enough}

% We propose a solution called \sys to assist data scientists in the EDA process. Given an exploratory step (e.g., filter, group-by, join) performed on a certain input dataframe, \sys{} generates corresponding explanations as follows (See Figure~\ref{fig:framework} for an illustration).
\subsection*{Overview of \sys}
Given an exploratory step (e.g., filter, group-by, join) performed on a certain input dataframe, \sys{} generates corresponding explanations as follows (See Figure~\ref{fig:framework} for an illustration).

\paratitle{Interestingness evaluation of dataframe columns} 
% Given the dataframe obtained from an analysis step, \sys{} first assesses the interestingness of each column in the given dataframe using measures that capture aspects of exceptionality~\cite{ex} and diversity~\cite{bla}. This allows us to detect the most interesting facets of the resulted dataframe in the context of the operation.
Given the results dataframe obtained from an exploration step, \sys{} first assesses the interestingness of each column in the dataframe using measures that are tailored for the specific exploratory operation. Herein, we employ measures capturing \textit{exceptionality}~\cite{sarawagi1998discovery} of filter/join steps and \textit{diversity}~\cite{hilderman2013knowledge} in group-by steps. This allows us to detect the most interesting facets of the resulted dataframe in the context of the operation.


\paratitle{Contribution calculation of input sets-of-rows}
As we show in our experimental evaluation (Section~\ref{sec:experiments}), highlighting  interesting aspects in the results is insufficient for understanding them and deriving concrete insights. Therefore, \sys{} detects meaningful subsets of the input dataframe that \textit{significantly contributes} to the interestingness score of one of the columns. 
Subsets of rows are used to provide concise explanations as proposed by previous work \cite{0002M13,RoyS14}. 
Our contribution measure draws on the notion of \textit{intervention}~\cite{pearl2009causality,0002M13}, and quantifies the influence of a set-of-rows from the input dataframe on an interestingness score by measuring how this score changes when we remove these rows. 

Traversing exponentially many sets of rows is infeasible, and furthermore some of these sets are more meaningful than others as explanations. We, therefore, introduce multiple partition methods that cluster the input rows by, e.g., their frequency of appearance, numeric binning, and many-to-one relationships, and use these methods to restrict the search to qualifying subsets.   

\paratitle{Skyline of explanation-candidates}
An explanation-candidate is defined by (1) a set-of-rows from the input dataframe, that contributes to the interestingness of (2) a certain column in the output dataframe. 
While thousands of such explanation-candidates typically exist, we are interested in the ones with \textit{high} contribution to columns with \textit{high} interestingness scores.
\system{} therefore scans the space of explanation-candidates, and using the skyline operator~\cite{borzsony2001skyline} retrieves only the \textit{dominating} ones, in terms of contribution and interestingness scores. 
Finally, for each such explanation-candidate, \sys{} generate a corresponding visualization, coupled with a coherent caption that highlights the interesting pattern derived from the given exploratory step. 

To allow for interactive performance for large databases, we incorporate a sampling optimization that is shown to be highly useful in practice.

% \ag{Amit: maybe add this here: ``To allow for interactive performance for large databases, we incorporate a sampling optimization that is shown to be highly useful in practice.''}

%Then, to surface insights, \sys{} detects what causes the dataframe to be interesting by identifying subsets of the input dataframe that significantly \textit{contributed} to each interestingness score. Our contribution measure draws on the notion of \textit{intervention}, first defined in the context of causality \cite{pearl2009causality,0002M13}.
%\amit{this should be clarified - what is a good explanation? which is both interesting and contributing}
%\amit{here explain that searching for ``good'' explanations requires scanning the explanation-candidates space} \amit{clarify that we have several measures, each corresponding to a different facet}
%To generate coherent, easy-to-follow explanations, rather than computing the contribution of arbitrary subsets of the data, \sys{} focuses its explanation only on \textit{meaningful} set-of-rows, obtained using multiple partition methods that cluster the input rows by, e.g., their frequency of appearance, numeric binning, and many-to-one relationships. 

%Next, \system{} scans the space of explanation-candidates (i.e, set-of-rows that contribute to a certain interestingness facet), and using the skyline-operator~\cite{skyline} retrieves only the \textit{dominating} ones, in terms of contribution and interestingness scores. 
%Finally, for each such explanation-candidate, \sys{} generate a corresponding visualization, coupled with a coherent caption that highlights the interesting pattern derived from the given exploratory step. 

\paratitle{Experimental evaluation}
% We implemented a prototype version of \sys{} \cite{repo} and performed an extensive set of experiments. 
We have implemented a prototype version of \sys{} \cite{repo} and performed a comprehensive user study and simulated experiments. 
The user study includes a detailed comparison of our approach to four baselines, both based on previous work and on explanations generated manually by experts. 
In our simulated experiments, we examine the scalability of our approach and further considered the usefulness of our optimization in aiding scalable performance while maintaining high accuracy. 
% \amit{AMIR - CAN YOU UPDATE THIS WITH A SUMMARY OF THE EXPERIMENTS PROCESS AND SHOW THE MAIN CONCLUSIONS?}

% \paratitle{Paper Outline}
\paragraph*{Paper Outline}
We begin with a survey of related work (Section~\ref{sec:related}),
then describe our data model for notebook-based dataframe exploration, and the process of generating and evaluating explanations (Section~\ref{section:algorithms}). 
% We then detail the architecture and components of \sys{} (Section~\ref{section:algorithms}),
We then present our experimental results in Section ~\ref{sec:experiments}. Finally, we conclude and discuss ideas for future work (Section~\ref{sec:conclusions}).

%returned to the user as an illustrating captioned-visualizations (Section~\ref{sec:skyline}), as illustrated in .

%\textit{dominating} ones by computing the skyline~\cite{skyline} in terms of contribution and interestingness.

%This results in a set of explanation-candidates containing 






%that with a significant \textit{contribution} to the interestingness score of $Q$ (Section~\ref{sec:contribution})

























==> model.tex <==
\section{EDA Explanation framework}\label{sec:model}

%Recall that our goal is to be able to take an EDA operation and explain, intuitively, what exactly is interesting about its results. 
While existing notions of interestingness, as discussed in Section~\ref{sec:prelim}, can assess the \textit{degree of interestingness} of an EDA operation -- it may be difficult to understand \textit{why} and \textit{what} exactly is interesting in the resulted dataframe. 

To that end, we suggest a framework for a refined interestingness analysis, that can detect the particular tuples that make the resulted dataframe interesting. As explained in the sequel, the sets of interesting tuples are then used to generate intuitive, natural language explanations of the interesting aspects of the resulted dataframe. 

In what comes next, we first provide a brief overview, then define the notion of tuple-bins, which are sets of semantically related tuples. We then define how to measure the contribution of a tuple-bin on the overall interestingness, and finally, we give a formal definition of our problem of generating EDA explanations. 


\paratitle{Overview.}
Recall from Section~\ref{sec:prelim} that Shapley values measure the contribution of an \textit{actor} to a \textit{value function} computed for a \textit{coalition} of actors. 
In our context, to measure what contributes to the interestingness of an EDA operation $\opr$ employed on a dataframe $\inputdf$ we use the Shapley formula in the following manner:

(1) actors, in our context, are tuple-bins, which are sets of semantically related tuples contained in $\inputdf$. (2) An actor coalition is a set of disjointed (i.e., non-overlapping) tuple-bins, and (3) the value function is a calculation of the interestingness of the EDA operation $\opr$ when employed on a specific tuples coalition. Finally, the Shapley value of a tuple-bin corresponds to its contribution to the interestingness of the operation $\opr$.  
\vspace{2mm}

We next detail our notions and definitions for calculating the interestingness contribution: We first define the tuple-bins and the value function, then provide the formal definition of the tuple-bins Shapley values.




%which are  cell-level interestingness, then extend the analysis to disjointed cell-sets. Last, we give a formal definition of our problem of generating EDA explanations. 

%\amir{Decide if we use bag or set semantics!}

\iffalse
\subsection{Cell-level Interestingness}
Intuitively, we define interesting cells as cells that \textit{contribute significantly} to the interestingness of their associated column.
We next explain how the contribution and its significance are measured.  


\vspace{1mm}
\paratitle{Cell Contribution.}
Given an EDA operation $\opr$ resulted in output dataframe $\outputdf$, attribute $A$ and interestingness score $I(q,A)$, we measure the contribution of each cell $\cell \in \acolumnout$ to the score $I(q,A)$ using the concept of Shapley values. 


We are interested in those cells that provide the maximum value to the interestingness score of $\disp_{out}$. 
We formalize the definition of a Shapley value of a tuple in a view w.r.t. an interestingness measure as follows. 
Shapley value is a concept borrowed from Game Theory \cite{...} and has been used in previous work to quantify the contribution of e.g. features of the data to the clasification \cite{...} and a tuple to a query result \cite{...}. In this paper, we use Shapley values to quantify the contribution of a cell to the interestingness of a dataframe, defined by the result of the given interestingness function. 

% \amit{as we discussed, since the operation q already contains the input/output dataframes you can remove it from the left-hand part of the equation below and just use Shap(c,q,I,A). Also as we remove c from the input, its better to define the removal of a cell beforehand, then use a notation like $q/c$} 

% For the next definition and in the sequel of the paper we will use the notation $\opr|_{S}$ to denote the dataframes composed of $S \subseteq \inputdf$ and $T \subseteq \outputdf$, where $S$ is the set of tuples that are the provenance of the tuples in $T$ according to $\opr$. For example, suppose we join tables $A$ and $B$, and we have $T \subseteq A \bowtie B$, then $S$ is the set of tuples from $A$ and $B$ that resulted in the tuples in $T$. 

For the next definition and in the sequel of the paper we will use the notation $\opr|_{S}$ to denote the dataframes composed of $S \subseteq \inputdf$ and $T \subseteq \outputdf$, where $T$ is the output of $\opr$ when given $S$ as input. For example, suppose we join tables $A$ and $B$, and we have $T \subseteq A \bowtie B$, then $S$ is the set of tuples from $A$ and $B$ that resulted in the tuples in $T$. 

\begin{definition}[Value function for Shapley value]
Given a subset of tuples from an input dataframe $S \subseteq \inputdf$, an operation $\opr$, and an interestingness measure $I$, the value function is 
$v(S):= I(\opr_S)$, where $\opr_S$ is the output dataframe generated from employing operation $\opr$ on the subset $S$.
%$I(T)$, where $T$ is the dataframe created by $\opr(S)$. We denote this function by $I(\opr_{S})$ to relate it to the input. 
\end{definition}


\begin{definition}[Shapley value of a tuple]\label{def:shapley_tuple}
Given an operation $\opr$ 
% resulting in the dataframe $\disp_{out}$ with the column $\disp_{out}[A]$, 
with the input dataframe $\disp_{in}$ and the column $\disp_{out}[A]$, 
and an interestingness measure $I$, the Shapley value of a tuple $t \in \disp_{in}$ is defined as:
\begin{scriptsize}
\begin{equation*}
% \begin{split}
Shap(t,\opr,I,A) = \sum_{\makebox[0pt]{$S\subseteq \disp_{in}{\setminus} \{t\}$}} \frac{|S|!(|\disp_{in}|-|S|-1)!}{|\disp_{in}|!}\cdot (v({S\cup \{t\}}) - v({S}))
% \end{split}
\end{equation*}
\end{scriptsize}
% Note that $\disp_{out}[A]$ represents a set of cells. \amit{this is already defined, see if the definition in section2 is good for you}
\end{definition}



The above definition intuitively says that the contribution of each tuple to the interestingness of the view is given by its contribution to the result of the interestingness function when considering all possible cell subsets. 

When $q$, $I$, and $A$ are clear from context, we refer to the contribution of a cell simply by $Shap(c)$.

Since the Shapely values are affected by the range of the particular interestingness measure (e.g., the range of divesity is unbounded while the range of exceptionality is bounded by $1$), we use a normalized form of the Shap value for each tuple by calculating its Z-score: 
% i.e., the number of standard deviations that the tuple's value is distant from the mean w.r.t its corresponding column:

\begin{equation*}
    \overline{Shap}(t) := \frac{Shap(t) - \mu}{\sigma}
\end{equation*}

\amit{maybe change the notation to contribution C(t)}




\begin{example}
\amir{Meet with Amit Mualem and decide what intermediate results do we needfor this example. we want to show the general flow of the computation: To calculate the shap value of an element, we need to remove it from the original table, calculate the interestingness with and without it. it would be good to show that in the example, rather than exemplifying the formula. }
\end{example}


\begin{comment}
\vspace{1mm}
\paratitle{Cell Significance.}
Since we are interested in cells that are prominent to the interestingness, in addition to the \textit{absolute} contribution of a cell we also measure its \textit{relative} significance.
Intuitively, cells are considered significant if their contribution value is substantially greater than the contribution of other cells in the column.
We quantify this by considering the contribution Z-score, i.e., the number of standard deviations that the contribution (Shapely) value is distant from the mean cell contribution in the same column. 


\begin{definition}[Cell Significance]\label{def:significance}
Given a cell contribution value $Shap(c)$
w.r.t. operation $\opr$ and attribute $\attr$,
let $\mu$ and $\sigma$ be the mean and standard deviation contribution (resp.) over all cells $c \in \acolumnout$. We. define the significance of the cell $c$ as:

\begin{footnotesize}
\end{footnotesize}
\end{definition}


\begin{example}
\amir{Show 2 cells with about the same Shap value, but one with high significance and one with low significance, and explain why the first one is more useful as an explanation}
\end{example}
\end{comment}

\begin{comment}
\vspace{1mm}
\amit{ consider omitting or change the definition to be more abstract - a function that takes as input the three ingredients}
\paratitle{Final Cell Interestingness Calculation.}
finally, the cell-level interestingness of a cell $c \in \acolumnout$ is defined as
\begin{equation*}
I(c) = I(q,A)\cdot Shap(c)\cdot Sig(c)
\end{equation*}

Namely, the multiplication of: (1) The column's interestingness score $I(q,A)$, (2) the cell's contribution value $Shap(c)$, and (3) the cell's significance value $Sig(c)$.
\end{comment}
\fi

\subsection{Partitioning the Dataframe to Tuple-Bins}

Our goal is to identify which particular tuples contribute mostly to the interestingness score $I(q,A)$.
To do so, we will use a specialized notion of Shapley values, dedicated to our goal.





\paratitle{Tuple-bins.}
As mentioned above, we are interested in the contribution of tuple-bins, sets of semantically related tuples, to the overall calculation of the interestingness.
We particularly use tuple-bins rather than individual such tuples, since they allow us to surface higher-level patterns when generating explanations, as well as to reduce running times.   


\begin{definition}[Tuples Binning Partition]
\label{def:binning}
% Given a dataframe column $\outputdf[A]$ a partition of  $\outputdf[A]$ into disjoint sets of cells $B_1, \ldots, B_n$ is called binning. 
Given the input dataframe $\inputdf$, a partition of  $\inputdf$ into disjoint sets of tuples $\mathcal{B} = \{B_1, \ldots, B_n, \hat{B}\}$ is called a binning partition where $\hat{B}$ is a special bin called don't-care bin. 
\end{definition}

\amir{TO DO AmitM: add a short explanation for what goes into the don't care bin}
Intuitively, $\hat{B}$ contains all tuples that will not be part of the explanation and therefore can be ignored. 

\begin{example}\label{ex:bins}
% \amir{Use the filter operation view and demonstrate both categorical and numerical binning. Motivate don't-care bin!}
Reconsider the Spotify table in Figure \ref{fig:spotify} and the result of the filter operation in Figure \ref{fig:filter}.
Binning the tuples based on the Genre column using categorical binning results in a partition of the tuples into ones with genres pop, edm, rap, and rock. Another binning option is by acousticness which results in a partition based on intervals of the range $[0,1]$. \amir{AmitM, what are the `don't care' bins in these partitions?}
\end{example}

In this work we focus on three types of binning partitions.
However, any kind of binning method complying with Definition~\ref{def:binning} is naturally supported by our framework. 

All binning methods takes as input a number $n$, which predefines the number of bins for each attribute. This number is highly important as it affects the number of actors in our Shapley values calculation (See Definition~\ref{def:shapley_bin}).
In Section~\ref{?} \amit{complete} we explain exactly how $n$ is set in order to optimize both the explanations' quality and generation time. 

We use the following binning methods to divide a dataframe $\df$ into $n$ bins. 

\noindent\textbf{Numeric-Based Binning} Given 
a numeric attribute $A$, we divide the tuples in $\df$ according to their corresponding values in $\acolumn$ to $n$ bins of equal width, ranging between the minimum and the maximum values in $\acolumn$. \amit{change to equi-heightuy}

%\amit{why do we use equiwidth and not equi-height so the bins are balanced?} 

\vspace{1mm}
\noindent\textbf{Categorical-Based Binning}
For a categorical attribute $A$ we divide $\df$ to $n$ bins corresponding to the $n$ most prevalent values in $\acolumn$. We then assign the rest of the tuples, corresponding to the rest of the values in $\acolumn$, to the don't-care bin $\hat{B}$.

\vspace{1mm}
\noindent\textbf{Hierarchical Binning.} \amit{this is for group-by operations, we could employ the categorical and leave out all the small groups. Instead we try to find for the group-by}

If a gruopby is on columns $A$
 and $B$, either $A$ or $B$ can be the one-to-many. 
 
\amit{AM - how does this work?} 

\amit{ we may have more than one binning method applied. i.e, we can filter by the frequency-based binning, or by the numeric binning.}
 
 

Given an attribute $A$, we can divide the tuples in $\df$ according to an implicit hierarchy (i.e., many-to-one relationship) between $A$, and another column $A'$, if exists. 
Similarly to the categorical-based binning, we take the $n$ most prevalent values in $A'$ as bins, and assign the rest to the don't-care bin $\hat{B}$. 

% See an example below \amit{refer to the ongoing example}
\begin{example}
Example \ref{ex:bins} describes both a categorical-based binning on the Genre attribute and a numerical-based binning on the Acousticness attribute. 
\end{example}


\subsection{Measuring Tuple-Bins Contribution Using Shapley Values}
We next adapt the Shaply score to our framework of explanations using the interestingness of tuple-bins.

\paratitle{Tuple coalitions \& value function.}
As mentioned above, tuple-bins are the actors considered in our Shapely formula. Correspondingly, given a bin partition $B$, a \textit{coalition} $S$ can be any subset of the bins in $B$ which do not contain the don't-care bin $\hat{B}$, i.e., $S \subseteq \mathcal{B}\setminus\{\hat{B}\}$. 

\begin{example}
% \amir{Once we have the binning partition, we can add an example of a coalition}
Consider the binning partition in Example \ref{ex:bins} for genres. A coalition of bins is a set of bins, e.g., the set $S = \{pop, edm, rap\}$ form a coalition of tuples. 
\end{example}

Next, we use the notion of coalitions to define the value function is defined, where each bin coalition $S$ is assigned a value. 

\begin{definition}[Value function for bin Shapley value]
\label{def:valuefunc}

%Given a bin partition $\mathcal{B}$ 
%and a don't-care bin $\hat{B}$, a subset of bins from an input dataframe

%$S \subseteq \mathcal{B}$, an operation $\opr$, and an interestingness measure $I$, 
Given an EDA operation $\opr(\inputdf)$ resulted in dataframe $\outputdf$, an interestingness measure $I$, a 
binning partition $B$ of the input dataframe $\inputdf$ and a 
tuple coalition $S$,
the value function for $S$ is defined as follows.
\begin{center}
$v(S) =$ 
\(\begin{cases}
I(\opr((\bigcup\limits_{B\in S}B) \cup \hat{B})),  & S \neq \emptyset \\
0,  & \text{otherwise} 
\end{cases}\)
\end{center}
%where $\opr_S$ is the output dataframe generated from employing operation $\opr$ on the subset $S$.
\end{definition}
According to Definition~\ref{def:valuefunc}, the value function of a tuple coalition is equivalent to the interestingness score of the operation $opr$ and column $A$, when executed on an input display that only contains the tuples in each bin $B \subseteq S$ and the don't-care bin $\hat{B}$. 

Note that we have implicitly defined the set of players in the game as the {\em bins instead of the tuples}. This allows us to get a more comprehensive and general explanations while also making the computation more efficient (as we will show in the sequel).

After defining what are the actors, coalitions, and their value function in our settings, we can now properly define the Shapley value that will be used to measure the contribution of tuple-bins to the interestingness score. 

% To quantify the contribution of a bin,
% we adapt the Shapley formula to consider coalitions of bins instead of coalitions of individual cells. We next show the adapted formula for computing the Shapley value of a bin $B$, where the notation $\disp_{out}[A] \setminus \{B\}$ and $T\cup \{B\}$ refers to the dataframe column without all the tuples in bin $B$ and the set of tuples $T$ along with all the tuples in $B$, respectively.
\begin{definition}[Shapley value of a bin]\label{def:shapley_bin}
Let $\opr$ be an operation, let $\disp_{in}$ be the input dataframe, let $\disp_{out}[A]$ be a column in $\opr(\disp_{in})$, let $\mathcal{B}$ be a binning partition of $\disp_{in}$, and let $I$ be an interestingness measure. 
The Shapley value of a tuple-bin $B \in \mathcal{B}$ is defined as:
\begin{small}
\begin{equation*}
Shap(B,\opr,I,A) = \sum_{\makebox[0pt]{$S\subseteq \mathcal{B} \setminus \{S\}$}} \frac{|S|!(|\mathcal{B}|-|S|-1)!}{|\mathcal{B}|!}\cdot (v({S\cup \{B\}}) - v(S))
\end{equation*}
\end{small}
\end{definition}
% As the number of bins is strictly smaller than the number of individual cells, the contribution computation for bins is significantly faster. 

When $q$, $I$, and $A$ are clear from context, we refer to the contribution of a bin simply by $Shap(B)$.

Last, since we are interested in comparing the contribution of bins of multiple partitions and attributes, we need to standardize the individual Shapley values. The Shapley values are affected by the range of the value function, which can vary, in our case, according to the particular interestingness measure (e.g., the range of the diversity measure is unbounded while the range of exceptionality is bounded by $1$). We therefore use a normalized form of the Shapley value for each tuple-bin, by calculating its Z-score: 
% i.e., the number of standard deviations that the tuple's value is distant from the mean w.r.t its corresponding column:

\begin{equation*}
    \overline{Shap}(B) := \frac{Shap(B) - \mu}{\sigma}
\end{equation*}






\begin{example}
% \amir{Meet with Amit Mualem and decide what intermediate results do we need for this example. we want to show the general flow of the computation: To calculate the shap value of an element, we need to remove it from the original table, calculate the interestingness with and without it. it would be good to show that in the example, rather than exemplifying the formula. }
In Example \ref{ex:bins} we have demonstrated two bin partitions. The Shapley value of `edm' according to the first partition is approximately 0.22 while the Shapley value of the bin with acousticness $>0.92$ was approximately 0.23. The normalized Shapley values were 1.63 and 2, respectively. 
\end{example}




%\subsection{Binning Methods}


\subsection{Problem Definition}
%The explainability score of a bin $Exp(B)$ is a combination of the following three components: 
%Using the notions introduced thus far, we can now define the problem of finding the most suitable explanation candidates.

Naturally, to generate meaningful explanations we want to discover, on one hand, tuple-bins with \textit{high Shapley value}, as it means that they contribute significantly to the interestingness score of their associated attribute. On the other hand, we prefer tuple-bins that are associated with attributes that obtain \textit{high interestingness score}. 


We therefore define the problem of of finding suitable explanation candidates as finding the tuple bins on the skyline of (1) bin Shapley value and (2) column interestingness score.      

The formal definition is as follows:


\begin{definition}\label{def:problem}
Given an output dataframe $\outputdf$ with attributes generated by an operation $\opr$,
let $\mathcal{B}_\opr$ be the set of all bins in the output dataframe $\outputdf$.
We are interested in finding the Skyline set of bins $S_\opr$, out of all bins
in terms of interestingness, contribution and significance:
\[ \forall B \in S_\opr \nexists B' \in \mathcal{B}_\opr,  I(B') \geq I(B) \land \overline{Shap}(B') \geq \overline{Shap}(B)
\]

\end{definition}

%Given an output dataframe $\outputdf$ with attributes $A_1, \ldots, A_m$, generated by an operation $\opr$ and $k \in \mathbb{N}$, we are interested in finding the $B_1, \ldots, B_k$ bins from columns $\outputdf[A_1], \ldots, \outputdf[A_m]$ such that $B_1, \ldots, B_k$ have the maximum explainability score . 







\begin{example}
% \amir{Show the bins in the skyline and explain why they are incomparable, i.e., one as higher shap yet lower interestingness, etc. Show a graph?}
Reconsider the result of the filter operation in Figure \ref{fig:filter} and the two binning approaches based on the genre column and the acousticness column shown in Example \ref{ex:bins}. The former approach (genre column) has a higher interestingness score of 0.25 compared to 0.2 of the latter approach (acousticness column), while the Z-score of the latter approach is $\approx 2$ compared to $\approx 1.6$ of the former approach. Therefore, both approaches are in the skyline.
\end{example}

Naturally, Definition \ref{def:problem} poses several computational challenges, from finding the more appropriate interestingness function and attributes for the bin partition to computing the Shapley values and Z-score of the bins. We address these challenges in the next section.


==> model_new.tex <==
%\section{Model \& Problem Definition}
\section{Modelling Notebook-based EDA}
\label{sec:model}

\amit{move this to section 4 and say that we briefly define the datafrme exploratin in notebooks}
%\subsection{}

    As mentioned above, the notebook interface allows users to explore datasets interactively. The user typically loads into the interface one or more tables from an external source (e.g., a CSV file, spreadsheet, or an SQL query from a database server), then interacts with them by employing programmatic EDA operations, such as filter, group-by, aggregate, etc.
The results of EDA operations are returned to the user as \textit{dataframe objects}.
% A dataframe is equivalent to a relational table or view,
% containing a multiset of rows projected over a set of columns.
% Therefore, we use the standard notations of databases and relations. 
% %A Dataframe, denoted $\df$, comprising of rows $r \in \df$ projected over a set of attributes $\attrs$. 
% Each row $r \in \df$ represents either a tuple or a group (in case $\df$ is resulted from a group-by operation). Correspondingly, an attribute $\attr$ specifies either a table attribute, or an aggregated column. 
% Furthermore, we refer to a dataframe \textit{column} by $\acolumn$, i.e., the multiset of all rows' values associated with the attribute $\attr$ in dataframe $\df$. 

A dataframe $\df$ is equivalent to a single relational table or view, comprises of a multiset of rows projected over a schema $\mathcal{A}(\df)$. 

%each row $r \in d$ may represent either a tuple, or a group 

%= (\attr_1, \ldots, \attr_m)$, where $\attr_i$

%is an attribute name. The dataframe contains a multiset of rows projected over a set of columns.
%Therefore, we use the standard notations of databases and relations. 
%A Dataframe, denoted $\df$, comprising of rows $r \in \df$ projected over a set of attributes $\attrs$. 
Each row $r \in \df$ represents either a tuple or a group (in case $\df$ is resulted from a group-by operation). Correspondingly, an attribute $\attr \in \mathcal{A}(\df)$ specifies either a table attribute, or an aggregated column. 
Furthermore, we refer to a dataframe \textit{column} by $\acolumn$, i.e., the multiset of all rows' values associated with the attribute $\attr$ in dataframe $\df$. 

Once the dataset is loaded, the user begins to perform exploratory \textit{steps}. In each step she first chooses on or more input \textit{dataframes}
%Each EDA operation takes as input one or more \textit{dataframes}
, denoted
$\inputdfs = \inputdf^1,\inputdf^2, \dots$. On the input dataframes she  
then employs an exploratory operation $q$, represented by a set of parameters (
(e.g., the filter criteria, the type of join, etc.).
Employing $q$ over $\inputdfs$ results in a new \textit{output dataframe},
denoted by $\outputdf= q(\inputdfs)$.
We refer to a full exploratory step by $Q=(\inputdfs,q,\outputdf)$

%, i.e., the results of employing the EDA operation defined by $q$ on input dataframes $\inputdfs$. 

\vspace{2mm}
\amit{put it in example env, maybe shorten it a little}
For example, consider an exploratory step in which a \textit{filter} operation is employed on $\df_0$, the initial dataframe from our running example (See Figure~\ref{fig:spotify_filter}):  $$q_1=\{\text{opr:}\textit{`FILTER'},~\text{criteria:}(\textit{popularity}>65)\}$$  

This results in a new dataframe $\outputdf= q_1(\df_0)$ that contains the subset of rows that comply to the criterion of ``popularity$>$65''. The resulted dataframe $\outputdf$ can be store in a new variable to serve as an input dataframe for later EDA steps. 
Also, the group-by
operation from our running example, is specified as follows:
$$ \begin{aligned} q_2=\{\text{opr:}\textit{`GROUP-BY'},~\text{on:} \textit{year},~\text{agg:} (&\text{loudness:} \textit{mean}, \\ &\text{danceability:} \textit{mean}) \}
\end{aligned}
$$
The resulting dataframe, as depicted in Figure~\ref{fig:spotify_groupby}, shows the mean values for \textit{loudness} and \textit{danceability} per year.
Another example is a join operation, specified by: $$q_3= \{\text{opr:}\textit{`JOIN'},~\text{type:}\textit{`inner'}\}$$
Hence, $q_2(\df_1,\df_3)$ is the output dataframe of the inner join between $\df_1$ and $\df_3$. 

Last, note that our prototype implementation of \sys{} currently supports filter, group-by and join operation, but can naturally be extended to support, in a similar manner, more advanced EDA and OLAP operations such as \textit{pivot}, \textit{diff}, and \textit{roll-up}. 
%\ag{Not sure how to rephrase here but we need to explicitly say that, for now, we only support Filter, Join, and GB}

















\begin{comment}

\subsection{The Problem of EDA Explainability}

Recall that our goal is to explain why is an exploratory step interesting, 
by finding which particular rows in $\inputdfs$ \textit{cause} the operation $q$ to results in an interesting output dataframe $\outputdf$

%$Q=(\inputdfs,q,\outputdf)$ is interesting,

%, by finding which particular rows in $\inputdfs$ \textit{cause} it to be 

%why is a resulting dataframe $\outputdf$ of an EDA operation is interesting, by finding what particular rows in $\inputdfs$ \textit{cause} $\outputdf$ to be \textit{interesting}. 

We next describe our notions for  \textit{interestingness} of EDA steps and \textit{contribution} of rows, and how we use them to define the problem of EDA explainability.  
\vspace{1mm}


First, as the notion interestingness is known to be complex and multi-faceted, we use a multiple 
\textit{interestingness score functions} 
, denoted by $\mathcal{I}=I_1,I_2,\dots$,
to quantify the interestingness of
an exploratory step $Q=(\inputdfs,q,\outputdf)$.
Each function $I \in \mathcal{I}$ evaluates a different interestingness facet, and provides a \textit{high} numerical score I(Q) for steps with \textit{interesting} result dataframes, and a low score otherwise. We elaborate on the methods for interestingness evaluation in Section~\ref{section:interestingness}. \daniel{We need here examples for concrete interestingness functions}

%\amit{Change the interestingness input to be the triple Din, q and dout}
%\amit{Amir should we go with ``causality'' instead?} 
% Next, we utilize a \textit{contribution} function,  denoted by $C(R, I, \outputdf)$ \amir{I think the abstract def. of the function can be written here}, in order to quantify the contribution of a set-of-rows $R \subset \inputdfs$ to the interestingness score $I(\outputdf)$. 
% Intuitively, rows obtaining a high contribution score are the ones that make  $\outputdf$ interesting w.r.t the function $I$. We discuss the specific definition of contribution we use in our framework in Section~\ref{section:explainability}.

\paragraph*{Contribution}
Given an interestingness function $I$,
and an exploratory step $Q=(\inputdfs,q,\outputdf$)
we utilize a \textit{contribution} function in order to quantify the contribution of a set-of-rows $R \subset \inputdfs$ to the interestingness score $I(Q)$. 
Our definition of contribution draws on the notion of intervention, first defined in the context of causality \cite{pearl2009causality} to measure the change in the outcome when the state of the input changes. This notion was adopted by the database community for measuring the change in query results when some of the rows are absent \cite{meliou2010causality,0002M13,RoyS14}. 
In particular, our contribution function is defined as follows (following the notations in \cite{0002M13}):
$C(R, I, Q) = I(\inputdfs,q,\outputdf) - I(\inputdfs-R,q,\outputdf)$.
Intuitively, rows obtaining a high contribution score are the ones that make the exploratory step $Q$ interesting w.r.t. function $I$.
%$\outputdf$ interesting w.r.t the function $I$. 


 Finally, to determine the most prominent sets-of-rows that cause a step $Q$ to be interesting, we need to find all sets-of-rows that have a \textit{significant contribution} to \textit{high interestingness scores} obtained w.r.t. a measure $I \in \mathcal{I}$. \daniel{$C$ was defined for individual rows, not for sets.}

We balance interestingness and contribution using the skyline operator~\cite{skyline}, namely, we are interested in finding sets-of-rows that are not `worse' than others in terms of both contribution and interestingness score. \daniel{Not clear if the skyline is w.r.t. indiviudal rows or sets need a crisp definition.}

 

 More formally, we define the problem of EDA explainability as follows:

 %Using our notions for EDA operations, interestingness and contribution we can now formally define the general problem of EDA explainability.

 
 \begin{definition}
 \label{def:general}

 Given an EDA operation and resulted dataframe $\outputdf= q(\inputdfs)$, a set of interestingness functions $\mathcal{I}$ and
 a contribution function $C$,
  let $R_{in}$ be the power set of rows, containing all possible sets-of-rows in the input dataframes, i.e., $R_{in}= \mathcal{P}\left(\bigcup_{\df \in \inputdfs}\{r~|~r \in \df \}\right)$.
 We are interested in finding sets-of-rows $R \in \inputdfs$ such that: 
 
%  are interested in finding the Skyline $S_R$ of tuple-sets $R$ s.t. $R \in \inputdfs$, in terms of both interestingness and contribution:
\[ \underset{R \in R_{in},~I \in \mathcal{I}}{\operatorname{SKYLINE}} \left(C(R,I,\outputdf),I(\outputdf)\right) \]

%\[ \forall R \in S_R,i\in I~~ \nexists R' \in \inputdfs,  \sum_{r\in R} EXP(r,i,\outputdf) ~~ i(\outputdf) \geq I(\outputdf) \land \overline{Shap}(B') \geq \overline{Shap}(B)
%\]
 \end{definition}


Naturally, evaluating the skyline define above is infeasible \scream{This seems like a claim of NP-hardness? May depend on the influence function. Make formal or omit.} In Section~\ref{section:algorithms} 
we propose to focus only on sets-of-rows that are semantically meaningful, using several binning strategies. This allows us to generate better, more coherent explanations (see Figure~\ref{fig:explained_new}), and also retain interactive running times.

\end{comment}

==> model_older.tex <==
\section{model}\label{sec:model}
We now give the definitions that lay at the heart of the problem of explaining EDA notebooks. 



% \amit{I think that the def of Shapley for tuples is rather novel therfore should appear in the solution section}
{\bf Shapley values for view tuples:} 
Given a view $D_{in}$, an operation $\op$ and an interestingness measure $I$, the contribution of each tuple in the view $\disp_{out} = \op(D_{in})$  to its interestingness can be quantified using the concept of Shapley value. 
We are interested in those tuples that provide the maximum value to the interestingness score of $\disp_{out}$. 
We formalize the definition of a Shapley value of a tuple in a view w.r.t. an interestingness measure as follows. 
\begin{definition}[Shapley value of a cell]\label{def:shapley_tuple}
Given an EDA view $\disp_{out}$ and an interestingness measure $I$, the Shapley value of the tuple $e\in \disp_{out}$ is defined as:
\begin{scriptsize}
\begin{equation*}
% \begin{split}
Shap(\disp_{out},I,e) = \sum_{\makebox[0pt]{$S\subseteq \disp_{out} \setminus \{e\}$}} \frac{|S|!(|\disp_{out}|-|S|-1)!}{|\disp_{out}|!}\cdot (I(q, A, \disp_{out}|_{S\cup \{e\}}) - I(q, A, \disp_{out}|_{S}))
% \end{split}
\end{equation*}
\end{scriptsize}
Note that $\disp_i$ is represented as a set of elements. 
\end{definition}

The above definition intuitively says that the contribution of each tuple to the interestingness of the view is given by its Shapley value. 

\begin{example}
\amir{add}
\end{example}

{\bf Explainability and weighted interestingness score:} 
Recall that we aim to focus the attention of the user on the most interesting parts of the view, i.e., given an interestingness measure, we wish to incorporate the most interesting tuples according to this measure. 
If, however, there are no particularly interesting tuples, the measure for which we computed tuple influence may not be a suitable choice. 
We formalize this idea be considering the {\em variance} of the Shapley values. 

\begin{definition}[Explainability]\label{def:explainability}
Given a view $\disp_{out}$, generated from $D_{in}$, and an interestingness measure $I$, let $\vec{v_s}$ an a vector of shapley values of the result view bins, where each bin contains a set of tuples from $\disp_{out}$, we define the explainability of an $I$ as:
\begin{footnotesize}
\begin{equation*}
    Explainability(\vec{v_s}) := Var(\vec{v_s})
\end{equation*}
\end{footnotesize}
\end{definition}

It is highly important to compute the Shapley values in $\vec{v_s}$ with the normalized $I$, otherwise the results will be biased to the score with the higher values.
Given an interestingness measure $I$ and its explainability score, we define its weighted score as the product of both measures. This way we are able to choose interestingness measures that are also explainable.

\begin{definition}[Weighted interestingness score]\label{def:score}
Given a view $\disp_{out}$ and an interestingness measure $I$, let $\vec{v_s}$ an a vector of Shapley values of the tuples of $\disp_{out}$, we define the weighted interestingness score of $I$ as $Wscore(I) = I(q,A,\disp_{out}) \cdot Explainability(\vec{v_s})$, i.e., the product of the result of $I$ on the view and the explainability of the tuples according to $I$.
\end{definition}

\begin{example}
\amir{add}
\end{example}


{\bf Problem definition:} 
We are now ready to define the {\em view explanation} problem. 

\begin{definition}[View explanation problem]\label{def:problem}
Given a view $\disp_{out}$, a set of interestingness measures $\mathcal{S}_I$, and an integer $k$, 
find the $k$ tuples with the highest Shapley values according to the interestingness measure $I \in \mathcal{S}_I$ such that $I = arg\_max_{I' \in \mathcal{S}_I} Wscore(I')$. 
\end{definition}

\begin{example}
\amir{add}
\end{example}

==> prelim_new.tex <==
\section{Preliminaries}\label{sec:prelim}
We next review the fundamental concepts that are used in the paper, including EDA operations and interestingness measures. 

\subsection{EDA Operations Via Notebook Interfaces}
Notebook interfaces allow the user to perform programmatic EDA operations via the notion of Dataframe objects. 
A Dataframe is equivalent to a relational table or view,
containing a multiset of rows projected over a set of columns.
Therefore, we use the standard notations of databases and relations. 
A Dataframe, denoted $\df$, contains a multiset of rows $r \in \df$ projected over a set of attributes $\attrs$. 
Each row $r$ represents either a tuple or a group (in case $\df$ is resulted from a group-by operation). Correspondingly, an attribute $\attr$ specifies either a table attribute, or an aggregated column. 
Furthermore, we refer to a dataframe \textit{column} by $\acolumn$, i.e., the multiset of all rows' values associated with the attribute $\attr$ in dataframe $\df$. 

%When interacting with a dataset via a notebook interface,
%the user typically loads one or more tables from external sources (i.e., a CSV file, a spreadsheet, or a SQL query from a database server) into views, then interacts with them by employing EDA operations.

 
When interacting with a dataset via a notebook interface,
the user typically loads one or more tables from external sources (i.e., a CSV file, a spreadsheet, or a SQL query from a database server) into notebook dataframes, then interacts with them by employing EDA operations, such as filter, group-by, aggregate, etc.

In our model, an EDA operation $\opr$ comprises three parts:

\paratitle{Input Dataframe(s):} 
An operation is evaluated on one or more existing dataframes, denoted $\inputdfs = \inputdf^1,\inputdf^2, \dots$. In case there is only one input dataframe we simply refer to it as $\inputdf$. 

\paratitle{Specification Parameters:} 
These parameters specify which particular operation to employ, containing, e.g., filter conditions, columns to perform aggregations on, etc.).

\paratitle{Output Dataframe:}
Evaluating the operation, with the specific parameters on the input dataframe(s) yields a corresponding output dataframe $\outputdf$ which contains its results. 


\vspace{2mm}
For example, the filter operation $\df_2 \leftarrow$ \elem{FILTER}($\df_1$,criteria) generates a new dataframe $\df_2$ that contains the subset of rows in $\df_1$ that comply to the criteria parameter. 
Another example is a join operation 
$\df_4 \leftarrow$ \elem{JOIN}($\df_1,\df_3$,$\{\attr$, 'inner'$\})$, in which Dataframes $\df_1$ and $\df_3$ are inner-joinned on attribute $\attr$, and the results are contained in $\df_4$.

\amit{mention that we use q(\df) to denote the output dataframe of operating $\opr$ on a dataframe $\df$}



%In a common EDA scenario performed via a notebook interface, the user loads $k$ ($\geq 1$) tables of a given dataset into corresponding Dataframes, denoted $\disp_0,\disp_1,\dots, \disp_k$, then begins performing a series of EDA operations (e.g., FILTER, GROUP\_BY, etc).
%Each operation $q_t$, employed at step $t (\geq k)$,

%Common such operations are filter, group-by and join.
%After employing an operation, the user examine the resulted dataframe, and consider if and which operation to employ next, on any of the existing dataframes.  


%An EDA operation $\action$ 
In this work we focus on generating explanations for three common EDA operations: \elem{FILTER}, \elem{JOIN}, and \elem{GROUP-BY}.
In Section~(\amit{complete}) we explain how additional, advanced operations such as PIVOT and UNPIVOT can be supported as well.  


The example below illustrates an exemplar fraction of an EDA notebook.

\begin{example}
\amit{present the two operations and refer to the results in the corresponding tables.}
\end{example}






%
%\amit{exemplify the other operations as well}




%An EDA notebook created w.r.t. a given input dataset is defined as a sequence of views $\disp_0, \ldots, \disp_n$, where $\disp_0$ is the initial dataset. 
%Each view is modeled as a set of elements $\disp_i = \{e_1, \ldots, e_k\}$, where an element $e_i$ is either a tuple or a group (in case $v_i$ is grouped-by). Each element $e_i$ is a vector of values $(v_1, \ldots, v_t)$ over an attribute vector $Attr$. 
%To get $\disp_i$ from $\disp_{i-1}$ we use an EDA operations $q_{i}$. 



\subsection{Interestingness Evaluation of EDA Operations}


As explained in the sequel, in order to generate an explanation for an EDA operation $q$, we first perform an analysis of its \textit{interestingness}.

Measuring the interestingness of data analysis operations has been intensively discussed in previous work (See, for example, the surveys in~\cite{geng2006interestingness} and \cite{hilderman2013knowledge}). Correspondingly, multiple different interestingness measures are suggested, each typically considers a different aspect of interestingness, for a different class of operations. 


In this work, we consider an interestingness measure $I$ to be a function that evaluates the interestingness of an EDA operation $\opr$, with respect to an attribute $\attr$, contained in the operation's output dataframe $\outputdf$. 


The function $I$ takes as input the attribute $\attr$, and the operation $\opr$ (which includes, as explained above, its input and output dataframes)
and returns a real number 

$I(\opr,\attr) \in \mathbb{R}$ indicating how interesting is operation $\opr$ w.r.t. attribute $A$ (higher score indicates a more interesting result).\footnote{Some measures consider even more  additional information, such as a user's prior knowledge/belief. While our framework can be naturally extended to support such measures we omit them for the simplicity of presentation.} 

We focus in this work on three different measures, one for each type of EDA operation we support:

\paratitle{Exceptionality (Filter).}
Following~\cite{sarawagi1998discovery,van2010maximal,vartak2015s}, our exceptionality measure favors \elem{FILTER} operations that yield an output Dataframe which significantly \textit{deviates} from the input Dataframe.



To quantify such deviation, for a filter operation $q_f$ and an attribute $A$, the function $I$ measures the differences between the values of $\acolumnin$ and $\acolumnout$, which are the columns associated with attribute $\attr$ in dataframes $\inputdf$ and $\outputdf$ (resp.).
To do so, we use the Kolmogorov–Smirnov (KS) test : we define a column's probability distribution $Pr(\acolumn)$ to be the relative frequency of its values (i.e., for each value $v \in \acolumn$, $Pr(v)$ is the probability to choose $v$ uniformly at random). 
% To do so, we use the Kullback-Leibler (KL) divergence measure: for each value $v \in \acolumn$, we define $Pr(v)$ is the probability to choose $v$ uniformly at random. 
% A column's probability distribution $Pr(\acolumn)$ is then defined to be $\prod_{v\in \acolumn} Pr(v)$. 
We then calculate the exceptionality by:
\begin{center}
\(Exceptionality(\fopr, \attr) := KS(Pr(\acolumnin),Pr(\acolumnout))\)    
\end{center}

%\amir{This looks inconsistent with the notation $I(\attr,\inputdfs,\outputdf)$}

\paratitle{Diversity Measure (Group-by).}
Our diversity measure favors group-by operations that yield notable differences in the aggregated values. 
Following~\cite{hilderman2013knowledge}, we define the diversity of a group-by operation $q_g$, w.r.t. an attribute $\attr$ (in its output dataframe $\outputdf$) as: 
\[
Diversity(\gopr,\attr) := Var(\acolumnout)  
\]


\paratitle{Exceptionality (Join).}
We adapt the notion of exceptionality to evaluate the interestingness of join operations. Oftentimes in join operations, the resulted dataframe contains a different number of tuples than in the original dataframes, we measure the deviation in the value distribution of each attribute, before and after the join operation. 
Similar to the case of filter operations, we calculate the exceptionality using KS test, comparing each attribute in the output dataframe to the attribute in its originated input dataframe:

\begin{center}
\(Exceptionality(\jopr, \attr) := KS(Pr(\acolumnin) | \attr \in \inputdf,Pr(\acolumnout))\)    
\end{center}


\begin{example}
% \amit{Show an examlpe of one measure for two columns - one with high score and one with low score and explain why the lower one is less interesting and vice verca}
% \amit{We will use the filter operation, column loundness is the interesting one and column 'name' is the non-interesting}
% \amit{todo: Make the numbers more extereme} 
Consider the Spotify table in Figure \ref{fig:spotify} and the result of the filter operation in Figure \ref{fig:filter}. Using the exceptionality measure for the columns Genre and Name, we get that $Ex(q_f, Genre) = 0.25$ while $Ex(q_f, NAme) = 0.17$, where $Ex$ is short for $Exceptionality$. Thus, according to this measure, the Genre column is more interesting than the Name column. 
\end{example}


\paratitle{Shapley Values.}
\amir{Background on Shapley value. Update if necessary}
In Cooperative Game Theory, Shapley value \cite{shapley1953value} is a way to distribute the contribution of each player, assuming they cooperate. 
Let $N$ be a finite set of players and $v : 2^N \to \mathbb{R}$, $v(\emptyset) = 0$ be a characteristic function. $v$ maps sets of players to the joint worth they generate according to the game. 
The contribution of player $a$ to a coalition $S$ (such that $a \not\in S$) is defined by the change in $v$ due to $a$'s addition, i.e., $v(S \cup \{a\}) - v(S)$. The Shapley value of player $a$ is the average of this contribution over the possible different permutations in which the coalition can be formed. 
Intuitively, for any player $a$, this value is the sum of $a$'s contribution to a change in $v$ over any possible coalition, factored by the size of the coalition such that mid-sized coalitions (of such there exists more of) are factored with a lower contribution.

{\footnotesize
$$Shapley(N,v,a) = \mathlarger{\mathlarger{\sum}}_{S\subseteq N\setminus \{a\}} \frac{|S|!(|N|-|S|-1)!}{|N|!} \\ \cdot (v(S\cup \{a\}) - v(S))$$
}

Shapley value is the only distribution function that satisfies several natural properties. 
Some of the properties that this formula satisfies are (1) \emph{Efficiency}, i.e., that the sum of Shapley values of all players is equal to the gain of the grand coalition, (2) \emph{Symmetry}, i.e., the worth of two players should be the same if they contribute equally to all possible coalitions, (3) \emph{Dummy}, i.e., if a player does not contribute to any coalition its worth should be 0, (4) \emph{Linearity}, i.e., if two separate games are combined together, then the worth distribution of the combined game should be equal to the sum of distributions of both games separately.

==> solution.tex <==
\section{solution}\label{sec:model}
\amir{DO NOT READ THIS SECTION YET}
We propose a system that finds the most suitable interestingness measure, and generates an explanation using the operation, the view and the interestingness measure, using shapley values.
\subsection{Finding The Most Interesting Column}
We want to explain why a specific view is interesting by showing how one column is interesting from an objective/relative point of view. At the start- every column is a candidate.

{\bf Eliminating correlated columns:} Columns with high correlation with the subject column (such as the aggregation attribute for group-by operations, or the filter attribute for filter operations) tend to generate high interestingness score. While sometimes it might be insightful, it might be very obvious in other cases. For instance, two columns that describe the temperature, one in Celsius and one in Fahrenheit- Any explanation that focuses on the relation of those columns is redundant. Hence we ignore each column that have a high correlation (\(>=\) predefined threshold \(T=95\%\))

{\bf Finding the most suitable interestingness measure:} Different Interestingness measures have different values distribution. comparing them as-is will give wrong results, and maybe even predictable result each time, if some measure output values are always higher than other measures. Hence we have to normalize the scores to distribute the same, and just then compare them to find the highest interestingness measure w.r.t the current view. For this issue we use work done by \cite{Interestingness}, which suggest such approach of normalizing such interestingness measures.
If the column is not very explainable \amitm{define}, we pass to the next candidate with the highest interestingness score, and so on. The column picked after this process, named the most interesting column.

\subsection{Explaining Using Shapley Values}
{\bf computing shapley values:} In order to make explanations more insightful, If the column is numerical we bin the column to a constant number of bins. This way the explanation describe a group of close values and it's influence on the interestingness measure. For shapley value computation, We use the SHAP python library, using approximations such as Sampling and KerenlSHAP. The target function is the normalized interestingness measure over the most interesting column values in the result view (after binning).
\newline
Each interestingness measure may need special data to highlight the interesting aspect it describes, and each interestingness measure will lay the facts in different way. In order to generate an explanation, each interestingness measure needs an explaining method, that creates an NL explanation, using an NL pattern that it has to fill using the source and result views. 

{\bf Explaining Diversity Measure:} For diversity measure, the explaining method uses the next pattern for group-by operations: "Specifically , the major deviation occurs on the group
\{top\_group\_name\} where the \{attribute\} value
changed from \{value in \(V_{i-1}\)\} to \{value in \(V_i\)\}.". The fields are filled by the shapley values calculated, where "value" is the value with the highest shapley value (with the Diversity function as the target function).

{\bf Explaining Exceptionality Measure:} For Exceptionality measure, the explaining method uses the next pattern for filter operations: "current view shows high exceptionality, specifically, the major deviation occurs on the attribute \{top\_attribute\}. For instance- the probability of \{value\_with\_highest\_shapley\} was \{\(P_1\)\} and changed to \{\(P_2\)\}". Where \{\(P_1\)\} is the probability of \{value\_with\_highest\_shapley\} in the input dataframe, and \{\(P_2\)\} is the probability in the output dataframe.

{\bf Explaining Intersection Measure:} For Intersection measure, the explaining method uses the next pattern for join operations: "The current view is highly verbose. The intersection \{table\_1\}", \{table\_2\}" indexes is big, \{intersection\_size\_percentage\}\% of \{table\_1\} tuples intersect with the tuples in \{table\_2\}. the join operation added the following new attributes: \{table\_2\_attributes\}.

notice that in this measure there is no use in shapley values(every tuple/value contribution is binary-in the intersection or not).

==> to_do.tex <==
\section*{To Do}
%Interestingness: R1-D2,R1-D3,R1-D4,R1-D6, R2-D4
%Section Interestingness, 3.8

% novelty and related work: R1-D1,R1-D2, R2-D2,R5-D1


%Novely R2-D2, R1-D1
\begin{itemize}
    \item Intro - Amit
    \item Related Work - Amit
    \item Running Example - Amit
    \item Amir - Replace SHAP with counterfactual
    \item Preliminaries: Interestingness definitions, Counterfactual definitions,
    \item Section Solution Architecture: 
    \begin{itemize}
        \item framework figure (user performs a query -> system performs binning -> compute influence and interestingness for every bin in an attribute of the resulting view -> compute skyline -> convert to a graph + text explanation)
        \item binning definition (motivation for binning - summarize the influencing parts of the view and efficient runtime)
        \item Binning types: categorical, numerical (equi-width,equi-height), many-to-one (add a figure showing `influence on the x-axis and interestingness on the y-axis for several bins)
        \item define skyline in our setting
        \item how do we generate textual explanations and graphical explanation?
        \item problem definition: what is the input and output
        \item algorithm box: input, binning partition, compute the skyline, output explanations
    \end{itemize}
    \item Experiments Section:
    \begin{itemize}
        \item Add an experiment regarding the effect of bin size both on running time and on the quality of explanation
    \end{itemize}
    
\end{itemize}

% \begin{itemize}
%     \item Section prelim: supported operations, supported interestingness measures, EDA notebook background, Shapley value background
%     \item Section model: Shapley values for tuples in the view according to interestingness measures, tradeoff between explanability score and interestingness score, problem definition: find top-$k$ tuples according to Shapley value
%     \item Section solution: finding the right interestingness measure, computing Shapley values for the tuples, textual templates as explanations
%     \item Section optimizations \amir{To Do}
%     \item Extension: summarize interesting tuples as predicates 
%\end{itemize}

\eat{

\begin{figure}[h]
    % \vspace{-2mm}
    \centering
	\begin{footnotesize}
		\begin{subfigure}{1\linewidth}
		    \centering
    		\begin{tabularx}{\linewidth}{| c | X | c | c | X | c | c | c |}
    			\hline Acoust. & Artists & Danceability & Loudness & Name & Popularity & Genre \\
    			\hline 0.7 & James Arthur & 0.76 & -5.726 & Train Wreck & 88 & pop \\
    			\hline \vdots & \vdots & \vdots & \vdots & \vdots & \vdots & \vdots \\
    % 			\hline 0.69 & $75$ & $Owner$ & $1$ & ?\\
    % 			\hline 0.14 & $25$ & $Owner$ & $0$ & ?\\
    % 			\hline 0.3 & $25$ & $Owner$ & $1$ & ?\\
    % 			\hline 0.82 & $24$ & $Spouse$ & $0$ & ?\\
    % 			\hline 0.47 & $10$ & $Child$ & $1$ & ?\\
    % 			\hline 0.99 & $10$ & $Child$ & $1$ & ?\\
    % 			\hline 0.01 & $30$ & $Owner$ & $0$ & ?\\
    % 			\hline 0.05 & $30$ & $Owner$ & $1$ & ?\\
    % 			\hline 0.58 & $30$ & $Owner$ & $1$ & ?\\
    			\hline
    		\end{tabularx}
    		\caption{Spotify table}\label{fig:spotify}
		\end{subfigure}
        \begin{subfigure}{1\linewidth}
            \centering
    		\begin{tabularx}{\linewidth}{| c | X | c | c | X | c | c | c |}
    		    \hline Acoust. & Artists & Danceability & Loudness & Name & Popularity & Genre \\
    % 			\hline 0.7 & James Arthur & 0.76 & -5.726 & Train Wreck & 88 & pop \\
    % 			\hline \vdots & \vdots & \vdots & \vdots & \vdots & \vdots & \vdots \\
                \hline 0.7010	& James Arthur	& 0.760	& -5.726	& Train Wreck	& 88	& pop\\
            	\hline 	0.6950& James Arthur & 	0.501 & 	-7.398 & 	Say You Won't Let Go & 	92	& pop\\
            	\hline 0.1410 & 	James Arthur & 	0.628 & 	-4.785 & 	Impossible &	78 & 	pop\\
            	\hline 	0.3080 & 	James Arthur & 	0.696 & 	-6.164 & 	Can I Be Him & 	78 & 	pop\\
            	\hline 0.8230&	James Arthur&	0.296&	-9.538&	Falling Like The Stars&	76&	pop\\
            	\hline 0.4680&	Ariana Grande&	0.737&	-4.771&	positions&	96&	pop\\
            	\hline 0.0217&	Ariana Grande&	0.708&	-7.070&	goodnight n go&	71&	pop\\
            	\hline 0.0102&	50 Cent&	0.561&	-6.106&	Window Shopper&	67&	rap\\
            	\hline 0.5800&	Led Zeppelin&	0.338&	-12.049&	Stairway to Heaven - Remaster&	78&	rock\\
    		     \hline
    		\end{tabularx}
    		\caption{Filter by $Popularity > 65$}\label{fig:filter}
		\end{subfigure}
		\begin{subfigure}{1\linewidth}
            \centering
    		\begin{tabular}{| c | c | c |}
    		    \hline {\bf Artists} & {\bf Genre} & {\bf Popularity} \\
    % 			\hline \vdots & \vdots & \vdots \\
    			\hline 50 Cent & rap &	42 \\
                \hline Ariana Grande &	pop &	70.25 \\
                \hline Avril Lavigne &	edm &	42 \\
                \hline James Arthur &	pop &	82 \\
                \hline Led Zeppelin &	rock &	52.33 \\
                \hline Martin Garrix &	edm &	50 \\
    		     \hline
    		\end{tabular}
    		\caption{Group by $Artists, Genre$ with $mean(Popularity)$}\label{fig:groupby}
		\end{subfigure}
	\end{footnotesize}
	\caption{Spotify table and operations \amir{Complete tables with relevant tuples}}
	\label{fig:db_table}
	\vspace{-3mm}
\end{figure}
}

